Dzyaloshinskii-Moriya interaction in transport through single molecule transistors

The Dzyaloshinskii-Moriya interaction is shown to result in a canting of spins in a single molecule transistor. We predict non-linear transport signatures of this effect induced by spin-orbit coupling for the generic case of a molecular dimer. The conductance is calculated using a master equation and is found to exhibit a non-trivial dependence on the magnitude and direction of an external magnetic field. We show how three-terminal transport measurements allow for a determination of the coupling-vector characterizing the Dzyaloshinskii-Moriya interaction. In particular, we show how its orientation, defining the intramolecular spin chirality, can be probed with ferromagnetic electrodes.

==> mkpaper <==
#!/bin/bash
# Produce PS and PDF from manuscript "paper.tex" (default)
# SYNTAX: with optional name
#   mkpaper <paper-name>

if [ $# -eq "0" ] # No arguments
then
    x="paper";
else
    x=$1;
fi

if [[ -e $x.tex ]]; then

   ## Update citations
   # ???? figure out the path?
   #../../bib/mkbib;

   # Compile latex + bibtex
   #
   # This code gave trouble with test.tex in zwanzig-realtime
   # an error prevents ps2pdf being done
   # latex $x.tex && \
   # bibtex $x    > /dev/null && \
   # latex $x.tex > /dev/null && \
   # latex $x.tex > /dev/null && \
   # dvips -Ppdf $x.dvi -o $x.ps && \
   # ps2pdf -sPAPERSIZE=a4 $x.ps $x.pdf

    latex $x.tex 
    bibtex $x    > /dev/null 
    latex $x.tex > /dev/null 
    latex $x.tex > /dev/null 
    dvips -Ppdf $x.dvi -o $x.ps
    ps2pdf -sPAPERSIZE=a4 $x.ps $x.pdf

    # zip the ps !!!
    if [[ -e $x.ps.gz ]]; then
	rm $x.ps.gz
    fi
    if [[ -e $x.ps ]]; then
	gzip $x.ps
    fi

    # Echo error checks
    echo "#####################"
    grep Citation $x.log
    grep Reference $x.log

    # Clean up precisely (most) files produced:
    for ext in aux dvi blg log end; do
	rm $x.$ext;
    done
else
    echo "mkpaper: aborting, manuscript file "$x".tex not found."
fi

